Peekaboo: Text to Image Diffusion Models are Zero-Shot Segmentors

Recently, text-to-image diffusion models have shown remarkable capabilities in creating realistic images from natural language prompts. However, few works have explored using these models for semantic localization or grounding. In this work, we explore how an off-the-shelf text-to-image diffusion model, trained without exposure to localization information, can ground various semantic phrases without segmentation-specific re-training. We introduce an inference time optimization process capable of generating segmentation masks conditioned on natural language prompts. Our proposal, Peekaboo, is a first-of-its-kind zero-shot, open-vocabulary, unsupervised semantic grounding technique leveraging diffusion models without any training. We evaluate Peekaboo on the Pascal VOC dataset for unsupervised semantic segmentation and the RefCOCO dataset for referring segmentation, showing results competitive with promising results. We also demonstrate how Peekaboo can be used to generate images with transparency, even though the underlying diffusion model was only trained on RGB images - which to our knowledge we are the first to attempt. Please see our project page, including our code: https://ryanndagreat.github.io/peekaboo

==> figures__implicit.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}{0.65\linewidth}
		\includegraphics[width=\linewidth]{figures__implicit.png}
	\end{minipage}
\hspace{0.02\linewidth}
	\begin{minipage}{0.3\linewidth}
		\caption{\textbf{Implicit neural function:} We illustrate the architecture of the multi-layer perceptron (MLP) network used to represent the learnable alpha masks in parametric form. The number of layers in the network, $L=4$. Masks are converted to Fourier domain and encoded as vectors $\bu$ and $\bv$ which are in turn represented by the weights of the MLP network ($\phi$). We highlight that our loss functions are used only for updating the parameters of this neural network used to represent the alpha masks.}
		\label{fig:implicit}
	\end{minipage}
	% \vspace{-0.5em}
%	\vspace{-1.0em}
\end{figure*}

==> figures__per_class.tex <==
\begin{figure}[t]
	\centering
		\includegraphics[width=0.95\linewidth]{figures__COCO-per-class-iou.png}
	\includegraphics[width=0.95\linewidth]{figures__Pascal-per-class-iou.png}
	\vspace{-1em}
		\caption{\textbf{Per-Class IoU values:} We report results on RefCOCO-C (left) and Pascal VOC-C (right) on a per-class basis. For RefCOCO-C, text captions were used to segment, and results were categorized according to the class of the referred object.}
		\label{fig:per_class}
	% \vspace{-0.5em}
	\vspace{-1.0em}
\end{figure}

==> figures__vis_everyday.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{0.6\linewidth}
    \includegraphics[width=\linewidth]{figures__vis_appendix__ducks.png}
\end{minipage}
\hspace{0.01\linewidth}
\begin{minipage}{0.37\linewidth}
    \caption{\textbf{Real-world applications}:
    Our proposed \modelname is able to localize objects of interest in the real world from arbitrary captions. We highlight how each localization successfully captures the relevant region with a clear overlap over the object centroid. This is particularly useful in applications such as robotics where interaction with arbitrary objects defined by natural language can be valuable.}
    \label{fig:vis_ed}
\end{minipage}
% 	\vspace{-1em}

\end{figure}

==> figures__vis_ew.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=0.49\linewidth]{figures__vis_appendix__ew_01.png}
    \includegraphics[width=0.49\linewidth]{figures__vis_appendix__em_wf.png}
\end{minipage}

\caption{\textbf{Varying granularity}:
Another feature of \modelname is its ability to segment at differing granularity. While the model performance in such situations is quite sensitive to the caption, we highlight how subtle variations to the caption allows us to localize relevant regions of image accordingly.}
\label{fig:vis_ew}
% \vspace{-1em}
\end{figure}

==> figures__vis_more.tex <==
\begin{figure*}[t]

\begin{minipage}{\linewidth}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__001.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__002.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__003.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__004.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__010.png}
\end{minipage}
\begin{minipage}{\linewidth}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__005.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__006.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__007.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__008.png}
	\includegraphics[width=0.195\linewidth]{figures__vis_appendix__009.png}
\end{minipage}
\caption{\textbf{\modelname is truly open vocabulary}:
We illustrate examples where \modelname is able to localize various regions of interest defined by references from popular culture. All of these are examples where the model has been able to correctly localize (identified region centroid or high IoU with correct region). The caption below each image is used to generate the same color mask. 
An interesting behavior of our model is its localization to the region most defined by the accompanying text caption. For example, in the case of Emma Watson in the top row second figure, it is visible how \modelname localizes on her face and body instead of her frock (see \cref{fig:vis_ew} for more on this).
}
\label{fig:vis_more}
% 	\vspace{-1em}

\end{figure*}

